DRL-GAN: A Hybrid Approach for Binary and Multiclass Network Intrusion Detection

Our increasingly connected world continues to face an ever-growing amount of network-based attacks. Intrusion detection systems (IDS) are an essential security technology for detecting these attacks. Although numerous machine learning-based IDS have been proposed for the detection of malicious network traffic, the majority have difficulty properly detecting and classifying the more uncommon attack types. In this paper, we implement a novel hybrid technique using synthetic data produced by a Generative Adversarial Network (GAN) to use as input for training a Deep Reinforcement Learning (DRL) model. Our GAN model is trained with the NSL-KDD dataset for four attack categories as well as normal network flow. Ultimately, our findings demonstrate that training the DRL on specific synthetic datasets can result in better performance in correctly classifying minority classes over training on the true imbalanced dataset.

==> sections/99-contribution.tex <==
\section{Contribution}
\label{sec:contribution}

Through our work, the primary contributions of this paper \mbox{include}:
\begin{enumerate}
    \item Introducing a framework for combining the DRL and GAN techniques for the purpose of network intrusion detection. That is, we propose a framework that uses a DRL model for intrusion classification trained using both network traffic data generated by a GAN model as well as open-source network data.
    \item Effectively using a GAN model to generate tabular, non-continuous data. Network traffic data generally contains many categorical features, which are challenging to translate and make use of with GANs as they are primarily intended to work with continuous values. While a small amount of noise in continuous values will generally not heavily impact the final image, noise with categorical values can significantly change the resulting record, reducing the viability of the generated data.
\end{enumerate}
